Optimization of the ionization time of an atom with tailored laser pulses: a theoretical study

How fast can a laser pulse ionize an atom? We address this question by considering pulses that carry a fixed time-integrated energy per-area, and finding those that achieve the double requirement of maximizing the ionization that they induce, while having the shortest duration. We formulate this double-objective quantum optimal control problem by making use of the Pareto approach to multi-objetive optimization, and the differential evolution genetic algorithm. The goal is to find out how much a precise time-profiling of ultra-fast, large-bandwidth pulses may speed up the ionization process with respect to simple-shape pulses. We work on a simple one-dimensional model of hydrogen-like atoms (the P\"oschl-Teller potential), that allows to tune the number of bound states that play a role in the ionization dynamics. We show how the detailed shape of the pulse accelerates the ionization process, and how the presence or absence of bound states influences the velocity of the process.

==> Makefile <==
all:
	pdflatex maxi_ionization.tex
	pdflatex maxi_ionization.tex
	pdflatex maxi_ionization.tex
	bibtex maxi_ionization
	pdflatex maxi_ionization.tex
	bibtex maxi_ionization
	pdflatex maxi_ionization.tex
	pdflatex maxi_ionization.tex
#	pdflatex maxi_ionization.tex


clean:
	rm -f *.bcf *.xml *.bbl *.log *.aux *~ maxi_ionization.pdf *.end *converted-to.pdf *.blg maxi_ionizationNotes.bib

tar:
	mkdir -p source
	rm -f source/*
	cp Makefile maxi_ionization.tex maxi_ionization.pdf maxi_ionization.bib \
           maxi_ionization.aux maxi_ionization.bbl maxi_ionization.blg \
           maxi_ionization.end *.eps source
	tar -czvf source.tar.gz source

